Uni4D: A Unified Self-Supervised Learning Framework for Point Cloud Videos

Self-supervised representation learning for point cloud videos remains a challenging problem with two key limitations: (1) existing methods rely on explicit knowledge to learn motion, resulting in suboptimal representations; (2) prior Masked AutoEncoder (MAE) frameworks struggle to bridge the gap between low-level geometry and high-level dynamics in 4D data. In this work, we propose a novel self-disentangled MAE for learning expressive, discriminative, and transferable 4D representations. To overcome the first limitation, we learn motion by aligning high-level semantics in the latent space \textit{without any explicit knowledge}. To tackle the second, we introduce a \textit{self-disentangled learning} strategy that incorporates the latent token with the geometry token within a shared decoder, effectively disentangling low-level geometry and high-level semantics. In addition to the reconstruction objective, we employ three alignment objectives to enhance temporal understanding, including frame-level motion and video-level global information. We show that our pre-trained encoder surprisingly discriminates spatio-temporal representation without further fine-tuning. Extensive experiments on MSR-Action3D, NTU-RGBD, HOI4D, NvGesture, and SHREC'17 demonstrate the superiority of our approach in both coarse-grained and fine-grained 4D downstream tasks. Notably, Uni4D improves action segmentation accuracy on HOI4D by $+3.8\%$.

==> checklist.tex <==
\clearpage
\newpage
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
limit. 

Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
\begin{itemize}
    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
    \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
\end{itemize}

{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

IMPORTANT, please:
\begin{itemize}
    \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
    \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
    \item {\bf Do not modify the questions and only use the provided macros for your answers}.
\end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The main contributions and scope have been included in the abstract and introduction.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The discussion on the limitations of our work is stated in Sec.~\ref{limitation} and Appendix~\ref{more limitations}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: For the theoretical part designed in the network, we have made an appropriate description in Appendix \ref{theory}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Comprehensive experimental details necessary for reproducibility, including datasets and model configurations, are thoroughly detailed in Sec.~\ref{exp}  and Appendix~\ref{appendix:details}. These details collectively ensure that the main experimental results supporting the claim and conclusions of the paper can be independently reproduced.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We will release the codes, logs, pre-training and fine-tuning checkpoints after the acceptance of this paper. The training logs of the fine-tuning stage and a piece of code for the t-SNE visualization have been uploaded to the supplementary materials.
    \item[] Guidelines: 
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide comprehensive experimental details, including hyperparameters (such as learning rate, epochs, batch size, etc.), and the type of optimizer, meticulously outlined in Appendix \ref{appendix:details}, Sec.~\ref{fine-tuning}, and Sec.~\ref{pre}. Additionally, we conduct ablation studies to select experiment settings, with key ablations elaborated upon in Tab.~\ref{tab:appendix_hyperparameter_ablation} and Tab.~\ref{tab:parameters_all}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We report the performance in terms of mean accuracy, chamfer distance, and the cosine similarity in Sec.~\ref{exp}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We primarily executed all experiments relying on GPU resources, with details of the specific GPUs used provided in Sec.~\ref{exp}, and corresponding execution times reported in Tab.~\ref{tab:appendix_memory}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have carefully reviewed the NeurIPS Code of Ethics, and we affirm that the research conducted in our paper adheres to the NeurIPS Code of Ethics in every respect.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We present broader impacts of our work in Appendix~\ref{Broader Impact}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: To our knowledge, our work dose not at the risk of this issue.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We properly cite related works, codes and datasets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not release new assets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our experiments focus on point cloud video data and do not include crowdsourcing or involve research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}. % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The research presented in the paper does not involve human subjects or crowdsourcing experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> table.tex <==
MSR
\setlength{\columnsep}{5pt}%
\begin{wraptable}{r}{8.5cm}
\centering
\footnotesize
\caption{Action recognition accuracy ($\%$) on the MSR-Action3D dataset. $\dagger$ indicates pre-training on NTU.}
\label{tab:msr}
  \begin{tabular}{lcc}
    \toprule
    Method & Reference  & Accuracy \\
    \midrule
    \multicolumn{3}{c}{\textit{Supervised Learning Only}} \\
    \midrule
    MeteorNet~\cite{liu2019meteornet} & ICCV2019 & 88.50 \\
    kinet~\cite{Zhong_2022_CVPR} & CVPR2022 & 93.27 \\
    PSTNet~\cite{fan2021pstnet} & ICLR2021 & 91.20 \\
    PPTr~\cite{wen2022point} & ECCV2022 & 92.33 \\
    3DInAction~\cite{Ben-Shabat_2024_CVPR} & CVPR2024 & 92.23 \\
    MAMBA4D~\cite{liu2024mamba4defficientlongsequencepoint} & CVPR2025 & 92.68 \\
    P4Transformer~\cite{fan2021point} & CVPR2021 & 90.94 \\
    \midrule
    \multicolumn{3}{c}{\textit{with Self-Supervised Representation Learning}} \\
    \midrule
    PSTNet + PointCPSC~\cite{sheng2023point} & ICCV2023 & 92.68 \\
    PSTNet + CPR~\cite{sheng2023contrastive} & AAAI2023 & 93.03 \\
    PSTNet + PointCMP~\cite{shen2023pointcmp} & CVPR2023 & 93.27 \\
    \rowcolor{gray!10}
    P4Transformer + MaST-Pre~\cite{shen2023masked} & ICCV2023 & 91.29 \\
    \rowcolor{gray!10}
    P4Transformer + M2PSC~\cite{han2024masked} & ECCV2024 & 93.03 \\
    \rowcolor{gray!30}
    \textbf{P4Transformer + Uni4D} & - & \textbf{93.38} 
    \scriptsize (\textcolor{red}{+2.44}) \\  
    \rowcolor{gray!30}
    \textbf{P4Transformer + Uni4D$^\dagger$} & -  & \textbf{93.38} \scriptsize (\textcolor{red}{+2.44})\\
    \midrule
    \multicolumn{3}{c}{\textit{with Linear Probing}} \\
    \midrule
    \rowcolor{gray!10}
    P4Transformer + MaST-Pre~\cite{shen2023masked} & ICCV2023 & 63.80 \\
    \rowcolor{gray!10}
    P4Transformer + M2PSC~\cite{han2024masked} & ECCV2024 & - \\
    \rowcolor{gray!30}
    \textbf{P4Transformer + Uni4D} & - & \textbf{84.62} \scriptsize (\textcolor{red}{+20.82}) \\ 
    \bottomrule
  \end{tabular} % 这里正确结束 tabular
\vspace{-0.7cm}
\end{wraptable}


\begin{wraptable}{r}{8.5cm}
\vspace{-0.4cm}
\centering
\footnotesize
\caption{Action recognition accuracy ($\%$) on the MSR-Action3D dataset. $\dagger$ indicates pre-training on NTU.}
\label{tab:msr}
  \begin{tabular}{lcc}
    \toprule
    Method & Reference  & Accuracy \\
    \midrule
    \multicolumn{3}{c}{\textit{Supervised Learning Only}} \\
    \midrule
    MeteorNet~\cite{liu2019meteornet} & \scriptsize{ICCV2019} & 88.50 \\
    kinet~\cite{Zhong_2022_CVPR} & \scriptsize{CVPR2022} & 93.27 \\
    PSTNet~\cite{fan2021pstnet} & \scriptsize{ICLR2021} & 91.20 \\
    PPTr~\cite{wen2022point} & \scriptsize{ECCV2022} & 92.33 \\
    3DInAction~\cite{Ben-Shabat_2024_CVPR} & \scriptsize{CVPR2024} & 92.23 \\
    MAMBA4D~\cite{liu2024mamba4defficientlongsequencepoint} & \scriptsize{CVPR2025} & 92.68 \\
    P4Transformer~\cite{fan2021point} & \scriptsize{CVPR2021} & 90.94 \\
    \midrule
    \multicolumn{3}{c}{\textit{with Self-Supervised Representation Learning}} \\
    \midrule
    PSTNet + PointCPSC~\cite{sheng2023point} & \scriptsize{ICCV2023} & 92.68 \\
    PSTNet + CPR~\cite{sheng2023contrastive} & \scriptsize{AAAI2023} & 93.03 \\
    PSTNet + PointCMP~\cite{shen2023pointcmp} & \scriptsize{CVPR2023} & 93.27 \\
    \rowcolor{gray!10}
    P4Transformer + MaST-Pre~\cite{shen2023masked} & \scriptsize{ICCV2023} & 91.29 \\
    \rowcolor{gray!10}
    P4Transformer + M2PSC~\cite{han2024masked} & \scriptsize{ECCV2024} & 93.03 \\
    \rowcolor{gray!30}
    \textbf{P4Transformer + Uni4D} & - & \textbf{93.38} 
    \scriptsize (\textcolor{red}{+2.44}) \\  
    \rowcolor{gray!30}
    \textbf{P4Transformer + Uni4D$^\dagger$} & -  & \textbf{93.38} \scriptsize (\textcolor{red}{+2.44})\\
    \bottomrule
  \end{tabular} % 这里正确结束 tabular
\vspace{-0.cm}
\end{wraptable}

T-L
\setlength{\columnsep}{5pt}%
\begin{wraptable}{r}{8.5cm}
\vspace{-3mm}
\centering
\small
\caption{Gesture recognition accuracy $(\%)$ on NvGesture (NvG) and SHREC'17 (SHR). }
\label{tab:gesture}
  \begin{tabular}{lcc}
    \toprule
    Method & NvG & SHR\\
    \midrule
    FlickerNet~\cite{2019FlickerNet} & 86.3 & -\\
    PointLSTM~\cite{min_CVPR2020_PointLSTM}  & 85.9 & 87.6\\
    PointLSTM-PSS~\cite{min_CVPR2020_PointLSTM} & 87.3 & 93.1\\
    
    kinet~\cite{Zhong_2022_CVPR} & 89.1 & 95.2\\

    P4Transformer~\cite{fan2021point} & 87.7& 91.2\\
    \midrule
    \rowcolor{gray!10}
    P4Transformer + MaST-Pre~\cite{shen2023masked} & 89.3 & 92.4 \\
    \rowcolor{gray!20}
    \textbf{P4Transformer + Uni4D} & \textbf{89.6}\scriptsize (\textcolor{red}{+1.9}) & \textbf{93.8}\scriptsize (\textcolor{red}{+2.6})\\ 
    \bottomrule
  \end{tabular}
  \vspace{-0.3mm}
\end{wraptable}




























三合一表格 
\begin{figure}[t]
\centering

% ------------------ 左边 MSR 表格 ------------------
\begin{minipage}[t]{0.49\textwidth}
\centering
\scriptsize
\captionof{table}{Action recognition accuracy ($\%$) on the MSR-Action3D dataset. $\dagger$ indicates pre-training on NTU.}
\label{tab:msr}
\scalebox{0.9}{
\begin{tabular}{lcc}
\toprule
    Method & Reference  & Accuracy \\
    \midrule
    \multicolumn{3}{c}{\textit{Supervised Learning Only}} \\
    \midrule
    MeteorNet~\cite{liu2019meteornet} & ICCV2019 & 88.50 \\
    kinet~\cite{Zhong_2022_CVPR} & CVPR2022 & 93.27 \\
    PSTNet~\cite{fan2021pstnet} & ICLR2021 & 91.20 \\
    PPTr~\cite{wen2022point} & ECCV2022 & 92.33 \\
    3DInAction~\cite{Ben-Shabat_2024_CVPR} & CVPR2024 & 92.23 \\
    MAMBA4D~\cite{liu2024mamba4defficientlongsequencepoint} & CVPR2025 & 92.68 \\
    P4Transformer~\cite{fan2021point} & CVPR2021 & 90.94 \\
    \midrule
    \multicolumn{3}{c}{\textit{with Self-Supervised Representation Learning}} \\
    \midrule
    PSTNet + PointCPSC~\cite{sheng2023point} & ICCV2023 & 92.68 \\
    PSTNet + CPR~\cite{sheng2023contrastive} & AAAI2023 & 93.03 \\
    PSTNet + PointCMP~\cite{shen2023pointcmp} & CVPR2023 & 93.27 \\
    \rowcolor{gray!10}
    P4Transformer + MaST-Pre~\cite{shen2023masked} & ICCV2023 & 91.29 \\
    \rowcolor{gray!10}
    P4Transformer + M2PSC~\cite{han2024masked} & ECCV2024 & 93.03 \\
    \rowcolor{gray!30}
    \textbf{P4Transformer + Uni4D} & - & \textbf{93.38} 
    \scriptsize (\textcolor{red}{+2.44}) \\  
    \rowcolor{gray!30}
    \textbf{P4Transformer + Uni4D$^\dagger$} & -  & \textbf{93.38} \scriptsize (\textcolor{red}{+2.44})\\
    \midrule
    \multicolumn{3}{c}{\textit{with Linear Probing}} \\
    \midrule
    \rowcolor{gray!10}
    P4Transformer + MaST-Pre~\cite{shen2023masked} & ICCV2023 & 63.80 \\
    \rowcolor{gray!10}
    P4Transformer + M2PSC~\cite{han2024masked} & ECCV2024 & - \\
    \rowcolor{gray!30}
    \textbf{P4Transformer + Uni4D} & - & \textbf{84.62} \scriptsize (\textcolor{red}{+20.82}) \\ 
    \bottomrule
\end{tabular}
}
\end{minipage}
\hfill
% ------------------ 右边：NTU + Gesture 上下两个小表 ------------------
\begin{minipage}[t]{0.47\textwidth}

% ----- NTU 表格 -----
\begin{minipage}[t]{\linewidth}
\centering
\scriptsize
\captionof{table}{Accuracy $(\%)$ on NTU under end-to-end fine-tuning and semi-supervised settings.}
\label{tab:ntu}
\scalebox{0.85}{
\begin{tabular}{lc}
\toprule
    Method & Accuracy \\
    \midrule
    3DV-PointNet++~\cite{wang20203dv} & 84.8 \\
    3DV-Motion++~\cite{wang20203dv} & 84.5 \\
    PST-Transformer~\cite{fan2022point} & 91.0 \\
    kinet~\cite{Zhong_2022_CVPR} & 92.3 \\
    PSTNet~\cite{fan2021pstnet} & 90.5\\
    
    P4Transformer~\cite{fan2021point} & 90.2 \\
    \midrule
    %\textbf{P4Transformer + Uni4D} (50\% Semi-supervised) & \textbf{86.5} \scriptsize (\textcolor{red}{+5.3})\\
    \rowcolor{gray!10}
    P4Transformer + MaST-Pre~\cite{shen2023masked} (End-to-end Fine-tuning) & 90.8 \\
    \rowcolor{gray!20}
    \textbf{P4Transformer + Uni4D} (End-to-end Fine-tuning) & \textbf{90.7}\scriptsize (\textcolor{red}{+0.5})\\
    \midrule
    \rowcolor{gray!10}
    P4Transformer~\cite{fan2021point} ($50\%$ Semi-supervised) & 81.2 \\
    \rowcolor{gray!20}
    \textbf{P4Transformer + Uni4D} ($50\%$ Semi-supervised) & \textbf{86.5} \scriptsize (\textcolor{red}{+5.3})\\
    \bottomrule
\end{tabular}
}
\end{minipage}

\vspace{0.1cm} % 控制上下表格间距

% ----- Gesture 表格 -----
\begin{minipage}[t]{\linewidth}
\centering
\scriptsize
\captionof{table}{Gesture recognition accuracy $(\%)$ on NvGesture (NvG) and SHREC'17 (SHR).}
\label{tab:gesture}
\scalebox{0.85}{
\begin{tabular}{lcc}
\toprule
    Method & NvG & SHR\\
    \midrule
    FlickerNet~\cite{2019FlickerNet} & 86.3 & -\\
    PointLSTM~\cite{min_CVPR2020_PointLSTM}  & 85.9 & 87.6\\
    PointLSTM-PSS~\cite{min_CVPR2020_PointLSTM} & 87.3 & 93.1\\
    
    kinet~\cite{Zhong_2022_CVPR} & 89.1 & 95.2\\

    P4Transformer~\cite{fan2021point} & 87.7& 91.2\\
    \midrule
    \rowcolor{gray!10}
    P4Transformer + MaST-Pre~\cite{shen2023masked} & 89.3 & 92.4 \\
    \rowcolor{gray!20}
    \textbf{P4Transformer + Uni4D} & \textbf{89.6}\scriptsize (\textcolor{red}{+1.9}) & \textbf{93.8}\scriptsize (\textcolor{red}{+2.6})\\ 
    \bottomrule
\end{tabular}
}
\end{minipage}

\end{minipage}

\vspace{-0.3cm}
\end{figure}














二合一
\begin{figure}[t]
\centering

% 左侧：NvG + SHR 表格
\begin{minipage}[t]{0.48\linewidth}
\centering
\scriptsize
\captionof{table}{Gesture recognition accuracy $(\%)$ on NvGesture (NvG) and SHREC'17 (SHR).}
\label{tab:gesture}
\scalebox{1}{
\begin{tabular}{lcc}
\toprule
Method & NvG & SHR\\
\midrule
FlickerNet & 86.3 & -\\
PointLSTM & 85.9 & 87.6\\
PointLSTM-PSS & 87.3 & 93.1\\
kinet & 89.1 & 95.2\\
P4Transformer & 87.7& 91.2\\
\midrule
\rowcolor{gray!10}
P4Transformer + MaST-Pre & 89.3 & 92.4 \\
\rowcolor{gray!20}
\textbf{P4Transformer + Uni4D} & \textbf{89.6}\scriptsize (\textcolor{red}{+1.9}) & \textbf{93.8}\scriptsize (\textcolor{red}{+2.6})\\ 
\bottomrule
\end{tabular}
}
\end{minipage}
\hfill
% 右侧：NTU 表格
\begin{minipage}[t]{0.48\linewidth}
\centering
\scriptsize
\captionof{table}{Accuracy $(\%)$ on NTU under end-to-end fine-tuning and semi-supervised settings.}
\label{tab:ntu}
\scalebox{0.75}{
\begin{tabular}{lcc}
\toprule
    Method & Accuracy \\
    \midrule
    3DV-PointNet++~\cite{wang20203dv} & 84.8 \\
    3DV-Motion++~\cite{wang20203dv} & 84.5 \\
    PST-Transformer~\cite{fan2022point} & 91.0 \\
    kinet~\cite{Zhong_2022_CVPR} & 92.3 \\
    PSTNet~\cite{fan2021pstnet} & 90.5\\
    
    P4Transformer~\cite{fan2021point} & 90.2 \\
    \midrule
    %\textbf{P4Transformer + Uni4D} (50\% Semi-supervised) & \textbf{86.5} \scriptsize (\textcolor{red}{+5.3})\\
    \rowcolor{gray!10}
    P4Transformer + MaST-Pre~\cite{shen2023masked} (End-to-end Fine-tuning) & 90.8 \\
    \rowcolor{gray!20}
    \textbf{P4Transformer + Uni4D} (End-to-end Fine-tuning) & \textbf{90.7}\scriptsize (\textcolor{red}{+0.5})\\
    \midrule
    \rowcolor{gray!10}
    P4Transformer~\cite{fan2021point} ($50\%$ Semi-supervised) & 81.2 \\
    \rowcolor{gray!20}
    \textbf{P4Transformer + Uni4D} ($50\%$ Semi-supervised) & \textbf{86.5} \scriptsize (\textcolor{red}{+5.3})\\
    \bottomrule
\end{tabular}
}
\end{minipage}

\vspace{-0.4cm}
\end{figure}


三合一
\begin{figure}[t]
\centering

% ------------------ 左边 MSR 表格 ------------------
\begin{minipage}[t]{0.49\textwidth}
\centering
\scriptsize
\captionof{table}{Action recognition accuracy ($\%$) on the MSR-Action3D dataset. $\dagger$ indicates pre-training on NTU.}
\label{tab:msr}
\scalebox{0.9}{
\begin{tabular}{lcc}
\toprule
    Method & Reference  & Accuracy \\
    \midrule
    \multicolumn{3}{c}{\textit{Supervised Learning Only}} \\
    \midrule
    MeteorNet~\cite{liu2019meteornet} & ICCV2019 & 88.50 \\
    kinet~\cite{Zhong_2022_CVPR} & CVPR2022 & 93.27 \\
    PSTNet~\cite{fan2021pstnet} & ICLR2021 & 91.20 \\
    PPTr~\cite{wen2022point} & ECCV2022 & 92.33 \\
    3DInAction~\cite{Ben-Shabat_2024_CVPR} & CVPR2024 & 92.23 \\
    MAMBA4D~\cite{liu2024mamba4defficientlongsequencepoint} & CVPR2025 & 92.68 \\
    P4Transformer~\cite{fan2021point} & CVPR2021 & 90.94 \\
    \midrule
    \multicolumn{3}{c}{\textit{with Self-Supervised Representation Learning}} \\
    \midrule
    PSTNet + PointCPSC~\cite{sheng2023point} & ICCV2023 & 92.68 \\
    PSTNet + CPR~\cite{sheng2023contrastive} & AAAI2023 & 93.03 \\
    PSTNet + PointCMP~\cite{shen2023pointcmp} & CVPR2023 & 93.27 \\
    \rowcolor{gray!10}
    P4Transformer + MaST-Pre~\cite{shen2023masked} & ICCV2023 & 91.29 \\
    \rowcolor{gray!10}
    P4Transformer + M2PSC~\cite{han2024masked} & ECCV2024 & 93.03 \\
    \rowcolor{gray!30}
    \textbf{P4Transformer + Uni4D} & - & \textbf{93.38} 
    \scriptsize (\textcolor{red}{+2.44}) \\  
    \rowcolor{gray!30}
    \textbf{P4Transformer + Uni4D$^\dagger$} & -  & \textbf{93.38} \scriptsize (\textcolor{red}{+2.44})\\
    \midrule
    \multicolumn{3}{c}{\textit{with Linear Probing}} \\
    \midrule
    \rowcolor{gray!10}
    P4Transformer + MaST-Pre~\cite{shen2023masked} & ICCV2023 & 63.80 \\
    \rowcolor{gray!10}
    P4Transformer + M2PSC~\cite{han2024masked} & ECCV2024 & - \\
    \rowcolor{gray!30}
    \textbf{P4Transformer + Uni4D} & - & \textbf{84.62} \scriptsize (\textcolor{red}{+20.82}) \\ 
    \bottomrule
\end{tabular}
}
\end{minipage}
\hfill
% ------------------ 右边：NTU + Gesture 上下两个小表 ------------------
\begin{minipage}[t]{0.47\textwidth}

% ----- NTU 表格 -----
\begin{minipage}[t]{\linewidth}
\centering
\scriptsize
\captionof{table}{Accuracy $(\%)$ on NTU under end-to-end fine-tuning and semi-supervised settings.}
\label{tab:ntu}
\scalebox{0.85}{
\begin{tabular}{lc}
\toprule
    Method & Accuracy \\
    \midrule
    3DV-PointNet++~\cite{wang20203dv} & 84.8 \\
    3DV-Motion++~\cite{wang20203dv} & 84.5 \\
    PST-Transformer~\cite{fan2022point} & 91.0 \\
    kinet~\cite{Zhong_2022_CVPR} & 92.3 \\
    PSTNet~\cite{fan2021pstnet} & 90.5\\
    
    P4Transformer~\cite{fan2021point} & 90.2 \\
    \midrule
    %\textbf{P4Transformer + Uni4D} (50\% Semi-supervised) & \textbf{86.5} \scriptsize (\textcolor{red}{+5.3})\\
    \rowcolor{gray!10}
    P4Transformer + MaST-Pre~\cite{shen2023masked} (End-to-end Fine-tuning) & 90.8 \\
    \rowcolor{gray!20}
    \textbf{P4Transformer + Uni4D} (End-to-end Fine-tuning) & \textbf{90.7}\scriptsize (\textcolor{red}{+0.5})\\
    \midrule
    \rowcolor{gray!10}
    P4Transformer~\cite{fan2021point} ($50\%$ Semi-supervised) & 81.2 \\
    \rowcolor{gray!20}
    \textbf{P4Transformer + Uni4D} ($50\%$ Semi-supervised) & \textbf{86.5} \scriptsize (\textcolor{red}{+5.3})\\
    \bottomrule
\end{tabular}
}
\end{minipage}

\vspace{0.1cm} % 控制上下表格间距

% ----- Gesture 表格 -----
\begin{minipage}[t]{\linewidth}
\centering
\scriptsize
\captionof{table}{Gesture recognition accuracy $(\%)$ on NvGesture (NvG) and SHREC'17 (SHR).}
\label{tab:gesture}
\scalebox{0.85}{
\begin{tabular}{lcc}
\toprule
    Method & NvG & SHR\\
    \midrule
    FlickerNet~\cite{2019FlickerNet} & 86.3 & -\\
    PointLSTM~\cite{min_CVPR2020_PointLSTM}  & 85.9 & 87.6\\
    PointLSTM-PSS~\cite{min_CVPR2020_PointLSTM} & 87.3 & 93.1\\
    
    kinet~\cite{Zhong_2022_CVPR} & 89.1 & 95.2\\

    P4Transformer~\cite{fan2021point} & 87.7& 91.2\\
    \midrule
    \rowcolor{gray!10}
    P4Transformer + MaST-Pre~\cite{shen2023masked} & 89.3 & 92.4 \\
    \rowcolor{gray!20}
    \textbf{P4Transformer + Uni4D} & \textbf{89.6}\scriptsize (\textcolor{red}{+1.9}) & \textbf{93.8}\scriptsize (\textcolor{red}{+2.6})\\ 
    \bottomrule
\end{tabular}
}
\end{minipage}

\end{minipage}

\vspace{-0.3cm}
\end{figure}




NTU\setlength{\columnsep}{5pt}%
\begin{wraptable}{r}{8.5cm}
\vspace{-0.4cm}
\centering
\scriptsize
\captionof{table}{Accuracy $(\%)$ on NTU under end-to-end fine-tuning and semi-supervised settings.}
\label{tab:ntu}
\scalebox{1}{
\begin{tabular}{lc}
\toprule
    Method & Accuracy \\
    \midrule
    3DV-PointNet++~\cite{wang20203dv} & 84.8 \\
    3DV-Motion++~\cite{wang20203dv} & 84.5 \\
    PST-Transformer~\cite{fan2022point} & 91.0 \\
    kinet~\cite{Zhong_2022_CVPR} & 92.3 \\
    PSTNet~\cite{fan2021pstnet} & 90.5\\
    
    P4Transformer~\cite{fan2021point} & 90.2 \\
    \midrule
    %\textbf{P4Transformer + Uni4D} (50\% Semi-supervised) & \textbf{86.5} \scriptsize (\textcolor{red}{+5.3})\\
    \rowcolor{gray!10}
    P4Transformer + MaST-Pre~\cite{shen2023masked} (End-to-end Fine-tuning) & 90.8 \\
    \rowcolor{gray!20}
    \textbf{P4Transformer + Uni4D} (End-to-end Fine-tuning) & \textbf{90.7}\scriptsize (\textcolor{red}{+0.5})\\
    \midrule
    \rowcolor{gray!10}
    P4Transformer~\cite{fan2021point} ($50\%$ Semi-supervised) & 81.2 \\
    \rowcolor{gray!20}
    \textbf{P4Transformer + Uni4D} ($50\%$ Semi-supervised) & \textbf{86.5} \scriptsize (\textcolor{red}{+5.3})\\
    \bottomrule
\end{tabular}
}\vspace{-0.7cm}
\end{wraptable}








\begin{figure}[t]
\centering

% 左侧：NvG + SHR 表格
\begin{minipage}[t]{0.48\linewidth}
\centering
\scriptsize
\captionof{table}{Accuracy $(\%)$ on NTU under end-to-end fine-tuning and semi-supervised settings.}
\label{tab:ntu}
\scalebox{0.75}{
\begin{tabular}{lcc}
\toprule
    Method & Accuracy \\
    \midrule
    3DV-PointNet++~\cite{wang20203dv} & 84.8 \\
    3DV-Motion++~\cite{wang20203dv} & 84.5 \\
    PST-Transformer~\cite{fan2022point} & 91.0 \\
    kinet~\cite{Zhong_2022_CVPR} & 92.3 \\
    PSTNet~\cite{fan2021pstnet} & 90.5\\
    
    P4Transformer~\cite{fan2021point} & 90.2 \\
    \midrule
    %\textbf{P4Transformer + Uni4D} (50\% Semi-supervised) & \textbf{86.5} \scriptsize (\textcolor{red}{+5.3})\\
    \rowcolor{gray!10}
    P4Transformer + MaST-Pre~\cite{shen2023masked} (End-to-end Fine-tuning) & 90.8 \\
    \rowcolor{gray!20}
    \textbf{P4Transformer + Uni4D} (End-to-end Fine-tuning) & \textbf{90.7}\scriptsize (\textcolor{red}{+0.5})\\
    \midrule
    \rowcolor{gray!10}
    P4Transformer~\cite{fan2021point} ($50\%$ Semi-supervised) & 81.2 \\
    \rowcolor{gray!20}
    \textbf{P4Transformer + Uni4D} ($50\%$ Semi-supervised) & \textbf{86.5} \scriptsize (\textcolor{red}{+5.3})\\
    \bottomrule
\end{tabular}
}
\end{minipage}
\hfill
% 右侧：NTU 表格
\begin{minipage}[t]{0.48\linewidth}
\centering
\scriptsize
\captionof{table}{Gesture recognition accuracy $(\%)$ on NvGesture (NvG) and SHREC'17 (SHR).}
\label{tab:gesture}
\scalebox{1}{
\begin{tabular}{lcc}
\toprule
Method & NvG & SHR\\
\midrule
FlickerNet & 86.3 & -\\
PointLSTM & 85.9 & 87.6\\
PointLSTM-PSS & 87.3 & 93.1\\
kinet & 89.1 & 95.2\\
P4Transformer & 87.7& 91.2\\
\midrule
\rowcolor{gray!10}
P4Transformer + MaST-Pre & 89.3 & 92.4 \\
\rowcolor{gray!20}
\textbf{P4Transformer + Uni4D} & \textbf{89.6}\scriptsize (\textcolor{red}{+1.9}) & \textbf{93.8}\scriptsize (\textcolor{red}{+2.6})\\ 
\bottomrule
\end{tabular}
}
\end{minipage}

\vspace{-0.4cm}
\end{figure}


\begin{table}[]
    \centering
    \caption{Ablation study on architecture designs.}
    \begin{tabular}{lccc}

\toprule
 & Acc (\%) ($\uparrow$) & CD $ \times  10^{-3}$ ($\downarrow$) & Cos ($\downarrow$) \\
\midrule
Recon only (one token) & 91.29 & \textbf{2.2} & - \\
Recon \& Align (one token) & 90.24 & 5.7 & 0.9991 \\
Recon \& Align (two tokens) & \textbf{93.38} & 4.3 & \textbf{0.2536} \\
\bottomrule
\end{tabular}
\label{tab:my_label}
\end{table}

\begin{figure}
    \centering
    \subfloat[w/o global alignment]{\includegraphics[scale=0.15]{LossCurve/LossWithoutGlobalv1.pdf}
	\label{fig:wo_global_loss} }
    \vspace{0.1cm}
    \subfloat[w/ global alignment]{\includegraphics[scale=0.15]{LossCurve/LossWithGlobalv2.pdf}
	\label{fig:w_global_loss} }
	\caption{The CE loss on MSR-Action3D during fine-tuning.}
	\label{fig:ab_global_loss} 
\end{figure}




\begin{table}
\centering
\small
\caption{Impact of temperature on MSR-Action3D. }
\label{tab:gesture}
  \begin{tabular}{cc}
    \toprule
    Temperature & Accuracy(\%)\\
    \midrule
    $[0.01,0.05)$ & 90.24\\
    $[0.05,0.1)$ & 91.98 \\
    $0.1$ & \textbf{93.38} \\
    \bottomrule
  \end{tabular}
\end{table}

\begin{table}
\centering
\small
\caption{Momentum parameter for the momentum encoder on MSR-Action3D. }
\label{tab:gesture}
  \begin{tabular}{cc}
    \toprule
    Momentum parameter & Accuracy(\%)\\
    \midrule
    $[0.99,0.995)$ & 85.36\\
    $[0.995,0.999)$ & 91.29 \\
    $0.999$ & \textbf{93.38} \\
    \bottomrule
  \end{tabular}
\end{table}


\begin{table}
\centering
\small
\caption{Queue Size on MSR-Action3D. }
\label{tab:gesture}
  \begin{tabular}{ccc}
    \toprule
     Size & Accuracy(\%)\\
    \midrule
    $6144$ & 90.94\\
    $12288$ & \textbf{93.38}\\
    $24576$ & -- \\

    \bottomrule
  \end{tabular}
\end{table}


\begin{table}
\centering
\small
\caption{Masking Ratio. }
\label{tab:mask ratio}
  \begin{tabular}{ccc}
\toprule
Model &Ratio & Accuracy(\%) \\
\midrule
C0 & 65\% & 91.99\\
C1 & 75\%& \textbf{93.38} \\
C2 & 85\%&  89.20\\
\bottomrule
\end{tabular}
\end{table}

\begin{table}
\centering
\small
\caption{Masking Strategy. }
\label{tab:mask strategy}
  \begin{tabular}{ccc}
\toprule
 Model &Strategy & Accuracy(\%) \\
\midrule
D0 & block & 88.94\\
D1 & video & 92.33 \\
D2 & frame & \textbf{93.38} \\
\bottomrule
\end{tabular}
\end{table}


\begin{equation} \label{attention}
\begin{aligned}
&Online\_Encoder: F_i=LayerNorms(\boldsymbol{E_{v}}),\\
&Momentum\_Encoder: F_i=LayerNorms(\boldsymbol{E}),\\
&Q=W_q\cdot F_i, \quad K=W_k\cdot F_i, \quad V=W_v\cdot F_i,\\
&\boldsymbol{Z}=Softmax\left(\frac{Q \cdot K^T}{\sqrt{D_k}}\right)\cdot V.
\end{aligned}
\end{equation}







\begin{table}[t]
\centering
\caption{Detailed experimental hyperparameters on datasets.}
\label{tab:parameters_all}
\scalebox{0.6}{
\begin{tabular}{c|ccccc}
  \toprule
  \textbf{Config} & \textbf{MSR} & \textbf{NTU} & \textbf{HOI4D} & \textbf{NvGestures} & \textbf{SHREC'17}\\
  \midrule
  pre-train optimizer & AdamW & Adamw & Adamw & - & -\\
  fine-tune optimizer & AdamW & AdamW & SGD & Adamw & Adamw\\
  pre-train learning rate    & 3e-4   & 3e-4   & 5e-4   & -     & -     \\
fine-tune learning rate    & 5e-4   & 5e-4   & 5e-2   & 5e-4  & 1e-3  \\
pre-train weight decay     & 5e-2   & 5e-2   & 1e-4   & -     & -     \\
fine-tune weight decay     & 1e-4   & 5e-2   & 1e-4   & 1e-4  & 1e-4  \\

  learning rate scheduler & cosine & cosine & cosine & cosine & cosine\\
  epochs (pre/ft) & 200 / 50 & 100 / 20 & 50 / 50 & - / 50 & - / 50\\
  batch size (pre/ft) & 96 / 48 & 56 / 48 & 4 / 8 & - / 24 & - / 24\\
  %\hline
  spatial radius $r_s$ (pre/ft) &0.3 / 0.7 & 0.1 / 0.1 & 0.9 / 0.9 & - / 0.1 & - / 0.3\\
  temporal stride $r_t$ & 2 & 2 & 1 & 2 & 2\\
  temporal radius $r_t$ & 3 & 3 & 3 & 3 & 3\\
  neighbor samples & 32 &32 & 32 & 16 & 9\\
  encoder's attention head \& depth & head = 8 \& depth=5 & head = 8 \& depth=10 & head = 8 \& depth=5 & head = 8 \& depth=10 & head = 8 \& depth=10\\
  momentum parameter & 0.999 & 0.999 & 0.999 & - & -\\
  queue Size & 12288 & 14436 & - & -& -\\
  decoder's attention head \& depth  & head = 8 \& depth=4 & head = 8 \& depth=4 &head = 8 \& depth=4 & - & -\\
  temperature & $\tau{=}0.1$ & $\tau{=}0.1$ & $\tau{=}0.1$ & - & -\\
  Few-shot / Semi-supervised lr & $0.0005$ & $0.0005$ & -& -& -\\
  input point cloud (pre/ft) &1024 / 2048 &1024 / 2048& 2048 / 2048 & - / 512& - / 256\\
  %down-sample & 32 & 32 & 2048 / 2048 & - / 512& - / 256\\
  \bottomrule
\end{tabular}
}
\end{table}

==> test.tex <==
\section{Introduction}
%Deep learning classifiers have achieved great success in pattern recognition tasks in numerous fields \citet{LeCun2015}.

Self-Supervised Learning (SSL) has has emerged as a promising approach in a variety of vision tasks \cite{he2020momentum, he2022masked, chen2020simple, kenton2019bert,tong2022videomae, feichtenhofer2022masked, PointContrast2020, pang2022masked}. These SSL-based frameworks have provided high-quality pre-trained models that exhibit enhanced performance and adaptability after fine-tuning on specific tasks. More recently, the success of SSL has extended to the domain of point cloud videos \cite{sheng2023contrastive,shen2023pointcmp,sheng2023point,zhang2023complete,shen2023masked}.

Although existing point cloud video SSL approaches have shown promise, there is still a lack of capacity to capture long-term motion representation essential for motion-aware downstream tasks~\cite{Liu_2022_CVPR}. As shown in Fig. \ref{fig:motivation}, MaST-Pre \cite{shen2023masked} produces inconsistent motion patterns between consecutive frames, indicating only short-term temporal dependencies. This method introduces a probabilistic modeling scheme that captures the dynamics in point tubes via temporal cardinality difference, which allocates points into octants of a sphere and calculates their angular distance to the octant central line. These hand-crafted features introduce an input-level motion inductive bias, however, are not conducive to learning transferable motion representations during self-supervised pre-training. Driven by this observation, we seek to model meaningful and decodable representations that allow high-fidelity reconstruction while containing expressive semantics, especially long-term motion representations to facilitate downstream fine-tuning.

\begin{figure*}[t]
    \centering
    {\includegraphics[width=1\textwidth]{Image/FIG1.png}}
	\caption{Comparison of the motion patterns for the action ``kick forward" after pre-training: (a) MaST-Pre presents segmented activations and inconsistent patterns; (b) Uni4D learns meaningful semantics and models long-term motion representation. }
	\label{fig:teaser} 
\end{figure*}

Our key inspiration is that the encoder-decoder bottleneck has provided a semantic-rich latent space \cite{preechakul2022diffusion, dong2022bootstrapped, jeong2024training}. This could be a suitable place for modeling high-level information, including the desired motion features. Intuitively, we can employ existing Masked AutoEncoders (MAE) \cite{dong2022bootstrapped,chen2022sdae,chen2024context} that perform predictions within the latent space and reconstruction in the pixel space simultaneously. However, due to the inherent complexity of 4D data, we find in practice that these methods fail to capture our desired meaningful representation features.

To address the above challenges, we propose the first \textbf{\textit{self-disentangled MAE}} for latent representation learning. This framework effectively disentangles different representation factors in a self-supervised manner, termed \textit{``self-disentangled"}. To capture \textit{low-level} geometric information, we train an MAE to reconstruct masked point tubes in the \textit{4D space}. On the other hand, \textit{high-level} semantic information is learned in the \textit{latent space}. We particularly focus on modeling two kinds of high-level semantics by two individual alignment modules: (1) bidirectional motion alignment to capture frame-level dynamics, and (2) global alignment to extract video-level temporal dependencies. Following \cite{chen2022sdae,dong2022bootstrapped,chen2024context}, we adopt a momentum encoder in parallel with the original MAE encoder to produce the latent prediction target. Nevertheless, the proposed self-disentangled MAE stands out for its superiority in eliminating the representation gap, e.g., the discrepancy between geometry and motion. This self-disentangled process is achieved by appending two different kinds of learnable tokens to the latent features before passing through the MAE decoder. One is the geometry token, prompting the decoder to conduct low-level geometric reconstruction. Another is the latent token, preventing the decoder from neglecting semantics when restoring low-level representations. This scheme is simple yet efficient, benefiting disentanglement between high-level and low-level features, which further provide a better alignment target between two encoders. In this case, the MAE encoder effectively models a latent space where latent features are discriminable in a self-supervised manner. We then introduce \textbf{\textit{Uni4D}}, a successful implementation of this framework for point cloud videos. We show that Uni4D, in the pre-training stage, has learned an expressive latent space with discriminative features. This could facilitate broader 4D tasks, covering action segmentation and action recognition that require different aspects of 4D representations. 

In conclusion, our contributions are summarized as:
% Although the geometric and semantic factors are modeled in separate spaces, the great discrepancy between the high-level and low-level information leads to significant model collapse during pre-training. 

\begin{itemize}
    \item We propose the first self-disentangled MAE to effectively model a latent space with discriminative representations, which yields Uni4D, a unified point cloud video framework suitable for fine-tuning on all 4D tasks.
    \item A novel bidirectional motion alignment module is designed to capture frame-level dynamics and a global alignment module to capture video-level semantics within the latent space for semantic modeling.
    \item Two kinds of learnable tokens are employed to disentangle high-level semantics against low-level features, thereby enabling effective training and representation learning in a self-supervised manner. 
    \item Uni4D achieves significant improvements over existing methods, achieving $+3.8\%$ segmentation accuract on HOI4D and $+2.44\%$ recognition accuracy on MSR-Action3D. Through extensive experiments, we show that the self-disentangled strategy provides valuable insights into model interpretability.
\end{itemize}

\section{Related Works}
\label{related works}

\textbf{Visual Mask Reconstruction}. The masked modeling mechanism has been shown great success in natural language processing~\cite{kenton2019bert,brown2020language}. Numerous computer vision tasks~\cite{bao2021beit,wang2022bevt, he2022masked} have adopted the Masked Auto-Encoder (MAE) to predict pixels from masked patches and significantly improve the fine-tuning performance \cite{chen2022sdae, dong2022bootstrapped,chen2024context}. This efficient self-supervised pre-training paradigm is subsequently adapted to video understanding ~\cite{tong2022videomae,feichtenhofer2022masked, wei2022masked, chen2022sdae}.

\textbf{Representation Learning for Point Clouds}. The representation of dynamic point clouds is essential for countless applications in computer graphics. Several voxel-based~\cite{luo2018fast,choy20194d,wang20203dv} and point-based~\cite{liu2019meteornet,fan2021pstnet,fan2021deep,fan2019pointrnn,min_CVPR2020_PointLSTM,fan2021point,fan2022point,wen2022point, Zhong_2022_CVPR, Ben-Shabat_2024_CVPR} representation learning algorithms have been developed. However, these methods rely heavily on the quality and scale of labeled datasets. Driven by the desire to eliminate expensive data annotations, the research community has investigated SSL for point cloud videos, such as contrastive learning \cite{radford2021learning, PointContrast2020,afham2022crosspoint} and masked reconstruction modeling~\cite{yu2021pointbert,pang2022masked,zhang2022point,liu2022masked,yan2024d}.

\textbf{Self-supervised Learning on Point Cloud Videos}. In the realm of point cloud videos, however, effective SSL frameworks for learning 4D representations are understudied. Early works \cite{sheng2023contrastive, shen2023pointcmp, sheng2023point, zhang2023complete} have primarily focused on the contrastive learning paradigm. The effectiveness of the masking strategy for point cloud videos is still underexplored. MaST-Pre~\cite{shen2023masked} and M2PSC~\cite{han2024masked} perform pre-training on masked dynamic point clouds. To learn the motion representation for point cloud video, they have proposed to predict the temporal cardinality difference or the motion trajectory, respectively. However, we notice that they possess two main limitations: (1) they require clumsy and time-consuming data pre-processing or feature extraction, and (2) both learn the motion directly from the decoded features, leading to short-term motion representation non-transferable for motion-aware downstream 4D tasks. In contrast, we resort to modeling the motion in latent space between the encoder-decoder architecture. We introduce the first self-disentangled MAE and demonstrate this innovative framework enables effective pre-training and models long-term motion representations.

\begin{figure*}[t]
    \centering
    {\includegraphics[width=0.96\textwidth]{Image/method_0313.pdf}}
	\caption{Overview of the Uni4D framework. We propose to model the motion and global information in the latent space. We leverage two kinds of learnable tokens to disentangle low-level and high-level features during decoding. The pre-trained model can provide a meaningful latent space where features are discriminable and transferable for downstream fine-tuning.}
	\label{fig:pipeline} 
\end{figure*}
\section{Methods}
\label{sec:Methods}

In this section, we introduce the proposed Uni4D, a novel self-disentangled MAE for point cloud videos. Our ultimate goal is to pre-train a motion-aware point cloud video encoder that learns meaningful and transferable representations for fine-tuning on broader 4D tasks. As illustrated in Fig. \ref{fig:pipeline}, Uni4D consists of an encoder-decoder structure to perform masking reconstruction, and an individual encoder to provide prediction target of latent. To capture expressive 4D representations, we propose to align high-level information in the latent space while restoring low-level information in the 4D space. In particular, we focus on modeling two high-level semantics: the frame-level motion representation and video-level global information. The self-disentangled learning ability is assured by two kinds of learnable tokens, which prevent feature entanglement and semantic diminishment during decoding. Without any hand-crafted design, Uni4D self-supervises the learning of discriminative 4D representations during pre-training.

\subsection{Masked Modeling}
Consider the input of a point cloud video as $\boldsymbol{P}\in \mathbb{R}^{L\times N\times 3}$, where $L$ is the sequence length and $N$ denotes the number of points in each frame. Following \cite{shen2023masked}, we construct the point tube sequence from the input point cloud sequence as:
\begin{equation}
    \boldsymbol{Tube}_{\hat{p}_i} = \{ p| p \in \boldsymbol{P}, S(p,\hat{p}_i)< r_s, T(p,\hat{p}_i)\leq \frac{r_t}{2}\}
\end{equation} 
where $\hat{p}_i$ is sampled from $p$ using Farthest Point Sampling (FPS), $S$ is the Euclidean distance, $T$ is the difference of two points in frame timestamps, $r_s$ and $r_t$ represent the spatial radius and the frame length in a tube, respectively. Next, these point tubes are projected to the full tube embeddings by Point 4D convolution (P4D)~\cite{fan2021point}, denoted as $\boldsymbol{E}$. 

To perform masked reconstruction, we randomly mask the point tubes using a high ratio (default to 75\%) to ease the learning of expressive representations and benefit the modeling of a meaningful latent space. The above process yields $N_v$ visible embeddings, denoted as $\boldsymbol{E}_{v}$.

\subsection{Architecture Design}
We propose the first self-disentangled MAE to learn discriminative representations suitable for 4D tasks. Following \cite{chen2022sdae, dong2022bootstrapped}, we adopt an encoder-decoder architecture to perform low-level reconstruction and a momentum encoder to benefit semantic modeling. In this section, we briefly discuss the network design and introduce the self-disentangled learning strategy in the next section. 

\textbf{Online Encoder}. The online encoder is implemented as a spatial-temporal Transformer~\cite{fan21p4transformer}, consisting of Multi-head Self-Attention (MAS), Layer Normalization (LN) and a MLP block in each layer $l$ as: 
\begin{equation}
f^{l}= MSA(LN(z^{l-1}))+z^{l-1}
\end{equation}
\begin{equation}
z^{l}= MLP(LN(f^{l}))+f^{l}
\end{equation}
This encoder only handles the visible visible embeddings, i.e., $z^0=\boldsymbol{E}_{v}$. For simplicity, we denote its outputs as $\boldsymbol{Z}_{v}\in\mathbb{R}^{L'\times N_v\times C}$, where $L'$ is the output length of P4D. 

\textbf{Decoder}. We employ a lightweight decoder $\mathcal{D}$ after the online encoder. To perform geometric reconstruction, we follow the paradigm of MAE \cite{he2022masked} and append several learnable tokens to represent masked point tubes, denoted as $\boldsymbol{T}_{geo}$. Our self-disentangled MAE differs from existing works as we further append a novel kind of learnable tokens, namely the latent tokens $\boldsymbol{T}_{lat}$, to preserve high-level features during decoding. Note that $\boldsymbol{T}_{geo}$ and $\boldsymbol{T}_{lat}$ are both appended to the visible embeddings $\boldsymbol{E}_v$ and passed through the same decoder. However, they are designed to prompt outputting low-level features and high-level features, thereby preventing the issue of feature entanglement raised by the decoder. After decoding, we apply a prediction head $\mathcal{H}$ to obtain the reconstructed results. 1D convolution is utilized to form this prediction head.
% The effectiveness of our disentanglement design is further substantiated in this module: the architecture of the regressor could be unprecedented shallow, e.g., one linear or 1D convolution, while previous works \cite{shen2023masked} adopted Transformer-based network to predict the masked data, either image, video, or point clouds.

\textbf{Momentum Encoder}. To learn the latent representation in a self-supervised manner, we are inspired by \cite{dong2022bootstrapped, chen2022sdae} to adopt a momentum encoder and update its weights from the online encoder using Exponential Moving Average (EMA). We input the unmasked full embeddings into the momentum encoder, i.e., $z^0=\boldsymbol{E}$, to ensure intact representation extraction. We denote the outputs of the momentum encoder as $\boldsymbol{Z}\in\mathbb{R}^{L'\times N'\times C}$.
% A recent work \cite{chen2024context} has a similar concern to prevent the entanglement of low-level and high-level features. However, it trains two separate decoders, which increases computation costs significantly and is extremely unreasonable for handling point cloud videos. Meanwhile, this simple yet effective design eased the representation learning and thereby enabling a lightweight implementation of this decoder. We provide more details of the decoder in Appendix X. 

\subsection{Self-Disentangled Learning Strategy}
\label{sec:self-disentangled strategy}
To achieve our goal of modeling meaningful 4D representations in the latent space. The propose of the self-disentangled learning strategy is based on an empirical finding: the latent space possesses rich high-level semantics, however, the decoder has raised the issue of feature entanglement and semantic diminishing due to the complexity of 4D representations. To address this, we leverage two kinds of learnable tokens: the geometry tokens $T_{geo}$ prompt the decoder to output low-level information for geometric reconstruction, while the latent tokens $T_{lat}$ prompt the decoder to preserve high-level semantics. 

\subsubsection{Low-level Learning Objective}
To conduct geometric reconstruction, we append the geometry tokens $\boldsymbol{T}_{geo}$ to the online encoder's outputs $\boldsymbol{Z}_v$ before passing through the decoder. Simply, we denote the decoder's outputs as $\boldsymbol{Z}_{geo}=\mathcal{D}(\boldsymbol{Z}_v,\boldsymbol{T}_{geo})$. We adopt the $l_2$ Chamfer Distance loss (CD) between the final predictions $\boldsymbol{P}_{rec}=\mathcal{H}(\boldsymbol{Z}_{geo})$ and the selected ground truth $\boldsymbol{P}_{gt}$ for learning low-level representations:
\begin{equation}
\label{eq:geometry_loss}
\begin{aligned}
\mathcal{L}_{geo} = \frac{1}{r_t}\sum^{r_t}_{i=1}\Bigg\{\frac{1}{\left|\boldsymbol{P}_{rec}^i \right|} \sum_{x \in \boldsymbol{P}_{rec}^i} \min_{y \in \boldsymbol{P}_{gt}^i} \|x - y\|^2 \\
    + \frac{1}{\left|\boldsymbol{P}_{gt}^i \right|}\sum_{y \in \boldsymbol{P}_{gt}^i } \min_{x \in \boldsymbol{P}_{rec}^i } \|y - x\|^2\Bigg\},
\end{aligned}
\end{equation}
where $r_t$ is the frame length in each tube.

\subsubsection{High-level Learning Objective}
Our high-level alignment target is to extract the frame-level consistent motion and video-level global representations, which is achieved by the following three objectives. 

\textbf{Latent Reconstruction}. We utilize the same decoder but append another kind of latent tokens $\boldsymbol{T}_{lat}$, yielding the outputs $\boldsymbol{Z}_{lat}=\mathcal{D}(\boldsymbol{Z}_v,\boldsymbol{T}_{lat})$. This design can effectively disentangle high-level semantics from low-level information without the necessity of introducing another decoder (see Sec.~\ref{sec:ab_architecture_design}). Intuitively, if the high-level information is preserved after decoding, this feature would have similar characteristics with the target latent, i.e., $\boldsymbol{Z}$. Therefore, the latent token $\boldsymbol{T}_{lat}$ should prompt the decoder to output features aligned with the latent embeddings. This latent alignment is achieved by:
\begin{equation}
\label{eq:latent_loss}
    \mathcal{L}_{lat} = 1-cos(MLP(\boldsymbol{Z}_{lat}),\texttt{stopgrad}(\boldsymbol{Z})),
\end{equation}
where $cos(\cdot)$ denotes the cosine similarity. Recall that the primary goal of this module is to prevent feature entanglement in the decoder. Therefore, a new MLP block is only applied to project the decoder's output $\boldsymbol{Z}_{lat}$ but no projection is used for the momentum encoder's output $\boldsymbol{Z}$. Meanwhile, we employ the stop-gradient operation \cite{chen2021exploring} to prevent collapsing of the momentum encoder.  

\textbf{Bidirectional Motion Alignment}. Different from the hand-crafted design in \cite{shen2023masked, sheng2023contrastive}, we aim to model the long-term motion representation in the expressive latent space. We compress the spatial information of two latent embeddings $\boldsymbol{Z}_v$ from the online encoder and $\boldsymbol{Z}$ from the momentum encoder by reshaping and max pooling. This yields two frame-level representations with shape $\mathbb{R}^{L'\times 1\times C}$, denoted as $\boldsymbol{H}_v=\{\hat{h}_1,\hat{h}_2,...,\hat{h}_{N'}\}$ and $\boldsymbol{H}=\{h_1,h_2,...,h_{N'}\}$, respectively. To model consistent motion patterns, we are inspired by \cite{zhang2023complete} and introduce a novel bidirectional motion alignment objective, formulated as:
\begin{equation}
\label{eq:motion_loss}
    \mathcal{L}_{motion} = - \frac{1}{B} \sum_{i=1}^{B} \log \frac{\exp\left(  MLP(\hat{h}_i) \cdot h_{j} / \tau \right)}{\sum_{k\neq j} \exp\left( MLP(\hat{h}_i) \cdot h_{k} / \tau \right)},
\end{equation}
where two individual MLP blocks are trained to project each frame in $\boldsymbol{H}_v$ to align with its target in $\boldsymbol{H}$ from forward and backward directions, respectively. We designate $i\in[2,N']$ and $j=i-1$ for the forward alignment, while $i\in[1,N'-1]$ and $j=i+1$ for the backward alignment. Similarly, the momentum encoder is not updated via gradient backpropagation from this objective.

\textbf{Global Alignment}. Despite our initial motivation to learn the motion within the latent space, we empirically find that solely modeling the motion leads to inferior fine-tuning performance on coarse-grained tasks (see Fig.~\ref{fig:ab_global_loss}). We are driven to extract global semantics in the latent space, i.e., the video-level information. To achieve this, we reshape $\boldsymbol{Z}_v$ to $\mathbb{R}^{L'\cdot N_v\times C}$ and $\boldsymbol{Z}$ to $\mathbb{R}^{L'\cdot N'\times C}$. Next, we apply the pooling operation and obtain $\hat{q}\in\mathbb{R}^{1\times C}$ and $q\in\mathbb{R}^{1\times C}$. To encourage the modeling of global representations, we align two embeddings by:
\begin{equation}
\label{eq:global_loss}
    \mathcal{L}_{global} = - \log \frac{\exp (MLP(\hat{q})\cdot q / \tau) }{ \sum_{k=0}^{K} \exp\left( MLP(\hat{q})\cdot q_k / \tau \right)},
\end{equation}
where $q_k$ denotes negative samples in a queue, $K$ is the queue length. We also apply the stop-gradient operation to the momentum encoder for this objective. 

\subsubsection{Overall Loss}
The final loss function is defined as:
\begin{equation}
    \mathcal{L}_{total} = \mathcal{L}_{geo} + \mathcal{L}_{lat} + \mathcal{L}_{global} + \mathcal{L}_{motion}.
\end{equation}

Since both low-level and high-level targets are involved in the above objectives, the encoder must produce discriminative representations for the decoder. It is only in this case that the decoder can disentangle the high-level semantics and the low-level geometric information with the help of two tokens. After pre-training, the MAE encoder models discriminative and transferable representations. This is exactly what its name indicates: a \textit{self-disentangled} MAE.
%Citations of inproceedings \cite{NIPS1994_24896ee4}.

%Citations of book \cite{bower2012book}.

%Citations of article \citep{Hasselmo5249}.
\section{Experiments}
In this section, we evaluate Uni4D from comprehensive aspects. Following~\cite{shen2023masked,shen2023pointcmp}, we compare to previous methods under end-to-end fine-tuning, semi-supervised learning, and transfer learning. We also investigate the few-shot learning ability of Uni4D. To demonstrate our superiority in learning good 4D representations, we focus on long-term point cloud videos on five benchmarks as MSR-Action3D~\cite{2010Action}, NTU-RGBD~\cite{shahroudy2016ntu}, HOI4D~\cite{Liu_2022_CVPR}, NvGestures~\cite{molchanov2016online} and SHREC'17~\cite{de2017shrec}, covering 4D action segmentation, action recognition, and gesture recognition. 

\begin{table}
\centering
\small
\caption{Action recognition accuracy ($\%$) on the MSR-Action3D dataset. $\dagger$ indicates pre-training on NTU.}
\label{tab:msr}
\scalebox{0.8}{ % 这里的括号是正确的
  \begin{tabular}{lcc}
    \toprule
      Method & Supervision & Accuracy \\
    \midrule
    MeteorNet~\cite{liu2019meteornet} & Supervised & 88.50 \\
    kinet~\cite{Zhong_2022_CVPR} & Supervised & 93.27 \\
    PSTNet~\cite{fan2021pstnet} & Supervised & 91.20 \\
    PPTr~\cite{wen2022point} & Supervised & 92.33 \\
    3DInAction~\cite{Ben-Shabat_2024_CVPR} & Supervised & 92.23 \\
    MAMBA4D~\cite{liu2024mamba4defficientlongsequencepoint} & Supervised & 92.68 \\
    P4Transformer~\cite{fan2021point} & Supervised & 90.94 \\
    PSTNet + PointCPSC~\cite{sheng2023point} & End-to-end Fine-tuning & 92.68 \\
    PSTNet + CPR~\cite{sheng2023contrastive} & End-to-end Fine-tuning & 93.03 \\
    PSTNet + PointCMP~\cite{shen2023pointcmp} & End-to-end Fine-tuning & 93.27 \\
    \midrule
    \rowcolor{gray!10}
    P4Transformer + MaST-Pre~\cite{shen2023masked} & End-to-end Fine-tuning & 91.29 \\
    \rowcolor{gray!30}
    \textbf{P4Transformer + Uni4D} & End-to-end Fine-tuning & \textbf{93.38} 
    \scriptsize (\textcolor{red}{+2.44}) \\  
    \rowcolor{gray!30}
    \textbf{P4Transformer + Uni4D$^\dagger$} & End-to-end Fine-tuning & \textbf{93.38} \scriptsize (\textcolor{red}{+2.44})\\
    \midrule
    \rowcolor{gray!10}
    P4Transformer + MaST-Pre~\cite{shen2023masked} & Linear Probing & 63.80 \\
    \rowcolor{gray!30}
    \textbf{P4Transformer + Uni4D} & Linear Probing & \textbf{84.62} \scriptsize (\textcolor{red}{+20.82}) \\ 
    \bottomrule
  \end{tabular} % 这里正确结束 tabular
}
\end{table}

\subsection{Pre-training}
\label{pre}
We evaluate our pre-trained feature representations on three datasets to substantiate the superiority of Uni4D in handling both short-term and long-term videos. As to short-term videos, we pre-train Uni4D for 200/100 epochs on MSR-Action3D/NTU-RGBD. Both datasets are densely sampled 24 frames and selected 1024 points in each frame. The frame sampling stride is set to 1/2 on MSR-Action3D/NTU-RGBD augmented with random scaling. We adopt P4Transformer~\cite{fan2021point} as our encoder for action recognition. As to long-term videos, we pre-train Uni4D for 50 epochs on HOI4D, with 150 frames densely sampled and 2048 points selected in each frame. We adopt PPTr~\cite{wen2022point} as our encoder for action segmentation. The decoder is implemented as a 4-layer Transformer for all datasets. The temperature $\tau$ is set to $0.1$ for Equ.~\ref{eq:motion_loss} and Equ.~\ref{eq:global_loss}. All experiments are conducted on GeForce RTX4090 $\times$ 2.

\begin{table}
\centering
\small
\caption{Action recognition accuracy $(\%)$ on NTU under end-to-end fine-tuning and semi-supervised settings. }
\label{tab:ntu}
\scalebox{0.85}{
  \begin{tabular}{lc}
    \toprule
    Method & Accuracy \\
    \midrule
    3DV-PointNet++~\cite{wang20203dv} & 84.8 \\
    3DV-Motion++~\cite{wang20203dv} & 84.5 \\
    PST-Transformer~\cite{fan2022point} & 91.0 \\
    kinet~\cite{Zhong_2022_CVPR} & 92.3 \\
    PSTNet~\cite{fan2021pstnet} & 90.5\\
    
    P4Transformer~\cite{fan2021point} & 90.2 \\
    \midrule
    %\textbf{P4Transformer + Uni4D} (50\% Semi-supervised) & \textbf{86.5} \scriptsize (\textcolor{red}{+5.3})\\
    \rowcolor{gray!10}
    P4Transformer + MaST-Pre~\cite{shen2023masked} (End-to-end Fine-tuning) & 90.8 \\
    \rowcolor{gray!20}
    \textbf{P4Transformer + Uni4D} (End-to-end Fine-tuning) & \textbf{90.7}\scriptsize (\textcolor{red}{+0.5})\\
    \midrule
    \rowcolor{gray!10}
    P4Transformer~\cite{fan2021point} ($50\%$ Semi-supervised) & 81.2 \\
    \rowcolor{gray!20}
    \textbf{P4Transformer + Uni4D} ($50\%$ Semi-supervised) & \textbf{86.5} \scriptsize (\textcolor{red}{+5.3})\\
    \bottomrule
  \end{tabular}
}
\end{table}

\subsection{End-to-end Fine-tuning}
We fine-tune the Uni4D pre-trained encoder with a linear classifier in a supervised manner to evaluate its end-to-end fine-tuning performance on NTU-RGBD,  MSRAction-3D, and HOI4D, respectively. Following~\cite{shen2023masked,zhang2023complete}, we use the same dataset for pre-training and fine-tuning.

\textbf{MSR-Action3D}. We use the same setting as ~\cite{fan2021point,fan2022point} during fine-tuning on this dataset. The recognition performance is reported in Tab. \ref{tab:msr}. Our pre-trained Uni4D significantly improves the baseline trained from scratch, increasing the accuracy rate from $90.94\%$ to $93.38\%$, and performs better than MaST-Pre with $+2.09\%$ accuracy. We also report the performance under linear probing. Out method outperforms MaST-Pre by $+20.82\%$ accuracy. Additionally, we evaluate Uni4D under a cross-dataset setting by pre-training on NTU-RGBD and then fine-tuning on MSR-Action3D. Interestingly, this model achieves the same score as when set to vanilla. From this, we speculate that Uni4D leverages the self-disentangled modeling scheme to learn good 4D representations. This can reduce dependence on dataset quality and scale as verified in the few-show learning experiment in Sec.~\ref{sec:few_show_learning}.

\textbf{NTU-RGBD}. We pre-trained our model for only 100 epochs due to the large scale of this dataset, but the results demonstrate the effectiveness of our method. As listed in Tab. \ref{tab:ntu}, Uni4D improves the baseline for $+0.5\%$ accuracy and obtains comparable performance to MaST-Pre that has been pre-trained for 200 epochs.
% While Uni4D obtains comparable performance, we verify its learning effectiveness.

It should also be noted that the above two datasets emphasize more on coarse-grained information \cite{Liu_2022_CVPR}. These datasets have relatively short videos. After downsampling, only a limited number of frames are needed to be recovered in the encoder. In this case, although modeling inconsistent motion patterns, MaST-pre~\cite{shen2023masked} still obtains a high score ($91.29\%$). We then demonstrate its incapability in processing long videos in the HOI4D dataset.

\textbf{HOI4D}. This dataset focuses on long-term video action segmentation at the fine-grained level, which is more challenging than the above two benchmarks. Tab. \ref{tab:hoi4d} reports the segmentation performance of our method following the setting in~\cite{zhang2023complete}. It is evident that Uni4D outperforms all models whether fully-supervised, self-supervised, or fine-tuned across all metrics. In particular, Uni4D gets $+3.6\%$ accuracy improvements and $+4.8\%$ F1 score at the overlapping threshold of $50\%$ over our baseline. On the other hand, other SSL methods present minor improvements. This comparison substantiates that the learned latent space of Uni4D has rich expressive semantics required for fine-grained understanding. We attribute this success to the self-disentangled learning strategy to discriminate between high-level semantics and low-level geometric representations. This provides a meaningful latent space where features are discriminable and transferable for comprehensive 4D tasks.

\begin{table}
\centering
\caption{Action segmentation performance on HOI4D. We report the frame-wise accuracy (Acc.), segmental edit distance (Edit), and segmental F1 scores at three levels of threshold.}
\label{tab:hoi4d}
\scalebox{0.68}{
  \begin{tabular}{lccccc}
    \toprule
    Method  & Acc. & Edit & F1@10 & F1@25 & F1@50 \\
    \midrule
    P4Transformer~\cite{fan2021point}  & 71.2& 73.1 &73.8& 69.2& 58.2\\
    C2P~\cite{zhang2023complete} & 73.5& 76.8& 77.2& 72.9 &62.4\\
    PPTr~\cite{wen2022point} & 77.4& 80.1 &81.7 
    &78.5 &69.5\\
    PPTr + STRL~\cite{2021Spatio} & 78.4& 79.1& 81.8 &78.6 &69.7\\
    PPTr + VideoMAE~\cite{feichtenhofer2022masked} & 78.6&  80.2 &81.9 &78.7 &69.9\\
    \midrule
    \rowcolor{gray!20}
    \textbf{PPTr + Uni4D} & \textbf{81.0}\scriptsize (\textcolor{red}{+3.6})& \textbf{82.5}\scriptsize (\textcolor{red}{+2.4}) &\textbf{84.6}\scriptsize (\textcolor{red}{+2.9})& \textbf{82.3}\scriptsize (\textcolor{red}{+3.8})& \textbf{74.3}\scriptsize (\textcolor{red}{+4.9})\\
    \bottomrule
  \end{tabular}
  }
  \vspace{-4mm}
\end{table}

\subsection{Semi-supervised Learning}
We also conduct semi-supervised fine-tuning experiments on NTU-RGBD. Following ~\cite{shen2023masked}, we use the full dataset during pre-training and then fine-tune with $50\%$ data for 20 epochs. We report the performance of Uni4D under semi-supervised learning in Tab. \ref{tab:ntu}. When reducing the scale of training data, it is more challenging for models to learn expressive 4D representations. Therefore, our baseline without pre-training fails to model discriminative features that are required for recognizing various actions. In contrast, our Uni4D pre-training facilitates the P4Transformer to produce superior accuracy with $+5.3\%$ improvements, which proves the effectiveness of our method.

\begin{table}
\centering
\small
\caption{Gesture recognition accuracy $(\%)$ on NvGesture (NvG) and SHREC'17 (SHR). }
\label{tab:gesture}
  \begin{tabular}{lcc}
    \toprule
    Method & NvG & SHR\\
    \midrule
    FlickerNet~\cite{2019FlickerNet} & 86.3 & -\\
    PointLSTM~\cite{min_CVPR2020_PointLSTM}  & 85.9 & 87.6\\
    PointLSTM-PSS~\cite{min_CVPR2020_PointLSTM} & 87.3 & 93.1\\
    
    kinet~\cite{Zhong_2022_CVPR} & 89.1 & 95.2\\

    P4Transformer~\cite{fan2021point} & 87.7& 91.2\\
    \midrule
    \rowcolor{gray!10}
    P4Transformer + MaST-Pre~\cite{shen2023masked} & 89.3 & 92.4 \\
    \rowcolor{gray!20}
    \textbf{P4Transformer + Uni4D} & \textbf{89.6}\scriptsize (\textcolor{red}{+1.9}) & \textbf{93.8}\scriptsize (\textcolor{red}{+2.6})\\ 
    \bottomrule
  \end{tabular}
\end{table}

\begin{table}
\centering
\caption{Accuracy ($\%$) of few-shot learning on MSR-Action3D. }
\label{tab:few-shot}
\scalebox{0.8}{
  \begin{tabular}{cccccc}
    \toprule
    \multirow{2}{*}{Method} & \multicolumn{2}{c}{\textbf{\textit{5-way}}} & & \multicolumn{2}{c}{\textbf{\textit{10-way}}} \\
    \cline{2-3}\cline{5-6}
    &\textit{1-shot}&\textit{5-shot}&&\textit{1-shot}&\textit{5-shot}\\
    \midrule
     MaST-Pre~\cite{shen2023masked}  & 70.2 & 95.7 && 71.1 & 92.7 \\
     \rowcolor{gray!20}
     Uni4D  & \textbf{74.5}\scriptsize (\textcolor{red}{+4.3}) & \textbf{97.8}\scriptsize (\textcolor{red}{+2.1}) && \textbf{79.4}\scriptsize (\textcolor{red}{+8.3}) &\textbf{95.8}\scriptsize (\textcolor{red}{+3.1}) \\
    \bottomrule
  \end{tabular}
  \vspace{-4mm}
}
\end{table}

\subsection{Transfer Learning}
To evaluate the generalization ability of Uni4D, we conduct experiments by transferring the pre-trained encoder to other datasets. Specifically, the encoder is first pre-trained on NTU-RGBD and then fine-tuned with a new classifier on NvGesture and SHREC'17, respectively. We use the same setup in Sec.~\ref{pre} during fine-tuning. This experiment is not only cross-dataset but also cross-task, as the model is pre-trained on action recognition while fine-tuned to perform gesture recognition. The results of recognition accuracy are presented in Tab.~\ref{tab:gesture}. Compared to another pre-training approach MaST-Pre, Uni4D better boosts the fine-tuning performance, as it gets $+1.9\%$ improvements on NvG and $+2.6\%$ on SHREC'17 over the baseline. This comparison substantiates Uni4D as a unified SSL framework for point cloud videos, effectively modeling discriminative and transferable representations to facilitate downstream tasks.

\subsection{Few-shot Learning}
\label{sec:few_show_learning}
To further demonstrate the generalization ability of our method, we also study the
model's capacity on few-shot learning. We have innovatively designed a few-shot dataset segmentation experiment tailored for 4D tasks. We adopt the \textit{``n-way m-shot"} settings from \cite{pang2022masked,yu2021pointbert}. For point cloud videos, the term \textit{``shot"} refers to one video and \textit{``way"} refers to one specific action, respectively. For example, \textit{``5-way 1-shot"} indicates the input of five actions, each action only has one video during training. To the best of our knowledge, we are the first to conduct such a few-shot learning experiment on 4D tasks.

Tab.~\ref{tab:few-shot} reports the few-shot learning performance of Uni4D compared to MaST-Pre. Each method is pre-trained on NTU followed by several few-show experiments on MSR. The proposed method exhibits dominant superiority for all settings. Uni4D obtains absolute improvements over MaST-Pre, indicating better one-shot and few-shot learning ability. Notably, Uni4D surpasses MaST-pre by $+8.3$ recognition accuracy under \textit{``10-way 1-shot"} as the strictest setting. This comparison fully demonstrates that the Uni4D framework is effective in extracting discriminative features.

\section{Ablation Studies}
\label{ablation}
In this section, we perform extensive ablations on Uni4D and empirically study our self-disentangled strategy. 

\begin{figure} [t]
	\centering
        \label{MSRvisualization}{
		\includegraphics[width =0.85\textwidth]{Image/Reconstructionv2.pdf} }\\
        
	\caption{Visualization of reconstruction results after pre-training.}
	\label{reconstruction} 
\end{figure}

\begin{figure} [t]
	\centering
        \label{MSRvisualization}{
		\includegraphics[width =0.9\textwidth]{Image/Reconlatent.pdf} }\\
        
	\caption{Performance comparison between models without (marked in orange) and with the latent reconstruction.}
	\label{ReconstrutionComparsion} 
\end{figure}    
\subsection{Visualization}
\textbf{Reconstruction Visualization}. In Fig.~\ref{reconstruction}, we provide two reconstruction examples of  Uni4D pre-trained on MSR-Action3D. We observe that Uni4D retains undesired noises when restoring the geometric information. We suspect the high-level features can affect the reconstruction accuracy due to the representation gap. \textbf{Does this mean that the network is not able to learn meaningful 4D representations?} To answer this, we further compare two models with and without the latent reconstruction on their pre-training and fine-tuning performance on MSR-Action3D. The comparison is shown in the Fig~\ref{ReconstrutionComparsion}. By removing the latent reconstruction objective, the model performs better on reconstruction but has lower accuracy on MSR-Action3D. In fact, our full model produces noisy reconstructions but has demonstrated superiority under fine-tuning. This finding provides valuable insights for understanding 4D representations and developing effective SSL approaches for point cloud videos: \textbf{the ultimate goal of pre-training is not to focus on better reconstruction accuracy but to capture meaningful spatial-temporal information for better fine-tuning performance}.  Nevertheless, low-level reconstruction still plays a critical role during fine-tuning, as the geometric structure is also essential for downstream tasks. This is evident in the comparison of B6 and B7 in Tab.~\ref{tab:ab_pretext}.

\begin{figure}[t]
    \centering
    {\includegraphics[scale=0.5]{Image/AttentionVis.pdf}}
	\caption{Attention activation comparison between two pre-trained encoder \textbf{without fine-tuning}. The top row is MaST-Pre \cite{shen2023masked} and the bottom row is our method. Observe that Uni4D presents consistent motion patterns and activations that match the target action.}
	\label{fig:attention} 
\end{figure}

\begin{figure}
	\centering
	\begin{subfigure}[b]{0.2\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Image/t-sne-baseline.png}
		\subcaption{MaST-Pre~\cite{shen2023masked}}
		\label{t-sne:MaST}
	\end{subfigure}
	\begin{subfigure}[b]{0.2\textwidth}
		\centering
		\includegraphics[width=1.0\textwidth]{Image/t-sne-ours.png}
		\subcaption{Uni4D}
		\label{t-sne:Uni4D}
	\end{subfigure}
	\caption{T-SNE results of Uni4D and MaST-Pre pre-trained on MSR-Action3D \textbf{without fine-tuning}.}
	\label{fig:t-sne} 
\end{figure}


\textbf{Attention Visualization}. As shown in Fig.~\ref{fig:attention}, we visualize the attention activations extracted from the pre-trained encoder. Unlike MaST-Pre, which produces inconsistent motion patterns (top row), by learning the motion and global semantics in the latent space, Uni4D captures long-term temporal dependencies (bottom row). More importantly, we observe that the pre-trained Uni4D has already shown interpretable representations according to the target action. For example, for the action \textit{``throwing high"}, the results of Uni4D highlight the hand area, which explains why it can facilitate downstream fine-tuning. 
% We verify this by fine-tuning for 5 epochs, whereas Uni4D gets $86.7\%$ recognition accuracy compared to the baseline $60.6\%$.

\textbf{Representation Visualization}.
\begin{wrapfigure}{r}{0.48\textwidth}
\vspace{-4mm}
\begin{center}
\includegraphics[clip,trim=0 0 0 0,width=0.23\textwidth]{Image/t-sne-baseline.png}
\includegraphics[clip,trim=0 0 0 0,width=0.23\textwidth]{Image/t-sne-ours.png}
\end{center}
\vspace{-3mm}
\caption{The test accuracy (\%) results obtained after training on the clean, UMT, and restoration datasets.}
\vspace{-2mm}
\label{fig:rev}
\end{wrapfigure}We use t-SNE to visualize the feature distributions of the pre-trained Uni4D and MaST-Pre for comparison. It is evident in Fig.~\ref{fig:t-sne} that the encoder, even without further fine-tuning, has already learned discriminative features, as clear boundaries can be observed between different categories.

\begin{table}[t]
	\caption{Ablation study on architecture designs.}
	\centering
	\label{table:ab_architecture}
	\resizebox{0.75\textwidth}{!}{
		\begin{tabular}{cccc}
			\hline
			& Latent Token & Single Decoder & Accuracy \\
			\hline
			A1  & - & $\checkmark$ &
			90.24 \\
			A2  & $\checkmark $ & - &
			90.94 \\
			\textbf{A3}  & $\checkmark $ & $\checkmark $ & \textbf{93.38} \\
			\hline
	\end{tabular}}
\end{table}

\begin{figure}
    \centering
    \subfloat[w/o global alignment]{\includegraphics[scale=0.15]{LossCurve/LossWithoutGlobalv1.pdf}
	\label{fig:wo_global_loss} }
    \vspace{0.1cm}
    \subfloat[w/ global alignment]{\includegraphics[scale=0.15]{LossCurve/LossWithGlobalv2.pdf}
	\label{fig:w_global_loss} }
	\caption{The CE loss on MSR-Action3D during fine-tuning.}
	\label{fig:ab_global_loss} 
\end{figure}

\subsection{Architecture Design}
\label{sec:ab_architecture_design}
We primarily discuss two of the most important architecture designs in Uni4D: (1) two kinds of learnable tokens to disentangle low-level and high-level features. (2) the same decoder to perform two reconstructions.

\textbf{Learnable Tokens}. Our proposed Uni4D adopts two distinct learnable tokens: geometry tokens to capture low-level characteristics and latent tokens to capture high-level semantics. This helps the network disentangle features. We ablate on this design by removing the latent tokens. The result is reported in Tab.~\ref{table:ab_architecture}. With latent tokens to disentangle high-level features, the performance of model A3 improves A1 from $90.24\%$ to $93.28\%$. This validates the use of two learnable tokens encourage the modeling of discriminative representations to facilitate action recognition.


\textbf{Decoder Design}
We then examine different decoder designs to perform two reconstruction tasks. We consider the following two designs to disentangle features: (1) two separate decoders dedicated to different reconstruction tasks, and (2) the simplest design of a single decoder. The results are presented in Tab.~\ref{table:ab_architecture}. Both models utilize two latent tokens, however, the two-decoder design does not lead to better performance. This ablation further verifies the effectiveness of two learnable tokens. Unlike \cite{chen2024context}, Uni4D is thereby allowed to adopt a lightweight decoder since the two tokens can prompt disentanglement of features.

\subsection{Global Alignment}
Uni4D models both motion and global representations as two high-level semantics. We claim that the global alignment module plays an important role in learning meaningful high-level 4D representations. We ablate this module and report the training and test losses during fine-tuning on MSR-Action3D in Fig.~\ref{fig:ab_global_loss}. Without global alignment, the pre-trained model lacks the ability to capture video-level representations. However, the model needs to discriminate long-term features to recognize actions. Therefore, it takes more training epochs to regain this ability, as the test loss is highly variable. Although this model has learned good motion representations during pre-training, we empirically find that it is not sufficient. This also highlights the complexity of 4D data: geometry and motion are not sufficient to represent all aspects of 4D representations.

\subsection{Self-Disentangled Modeling Strategy}
In Tab.~\ref{tab:ab_pretext}, we construct ablations of different pretext tasks on the MSR-Action3D dataset. Observing from the results of models B1 and B2, the introduction of latent reconstruction has shown significant degradation, While model B3 directly learns the motion in the latent space, and does not provide an expressive latent space to boost downstream fine-tuning. These two cases also indicate the complexity of 4D data with large discrepancies between low-level and high-level semantics. The model B4 indicates other semantics in the latent space, while the alignment between decoded features and latent features can diminish these semantics. On the other hand, the model B5 and B6 highlight the importance of geometry and motion information for 4D tasks, respectively, as they have no improvement on B1. The combination of all components yields remarkable improvements, which verifies our self-disentangled modeling strategy in learning meaningful 4D representations. 


\begin{table}
    \small
    \centering
  \caption{Ablation studies on different pretext tasks.}
  \label{tab:ab_pretext}
  \scalebox{0.85}{
  \begin{tabular}{cccccc}
    \toprule
    Model&$\mathcal{L}_{geo}$&$\mathcal{L}_{lat}$&$\mathcal{L}_{global}$&$\mathcal{L}_{motion}$&Acc.(\%)\\
    \midrule
    B1& $\checkmark $& $ $& $ $ & $ $&91.63\\
    B2& $\checkmark $& $\checkmark $& $ $ & $ $&85.36\\
    B3& $\checkmark $& $ $& $ $ & $\checkmark $&91.63\\
    B4& $\checkmark $& $\checkmark $& $ $ & $\checkmark $&90.94\\
    B5& $\checkmark $& $\checkmark $& $\checkmark $ & $ $&91.29\\
    B6& $ $& $\checkmark $& $\checkmark $ & $\checkmark $&91.63\\
    B7 (Ours)& $\checkmark $& $\checkmark $& $\checkmark $ & $\checkmark $&\textbf{93.38}\\
  \bottomrule
\end{tabular}
}
\end{table}

\section{Conclusion}
In this paper, we introduced Uni4D, the first self-disentangled MAE for point cloud video representation learning. Uni4D addresses key challenges in existing methods, effectively modeling long-term motion representations in a latent space while preserving geometric information in 4D space. To resolve the representation gap in 4D data, we introduce the latent tokens along with the geometric tokens to enable self-disentangled learning for high-level and low-level at the same time. Extensive experimental results on multiple 4D benchmark datasets demonstrate the effectiveness of Uni4D, particularly in long video processing, where it achieves significant performance gains. Our findings highlight the potential of the self-disentangled MAE structure for learning discriminative 4D representations, paving the way for future advancements in point cloud video understanding and disentanglement learning.


\begin{figure} [t]
	\centering
        \label{MSRvisualization}{
		\includegraphics[width =0.9\textwidth]{Image/Reconlatent.pdf} }\\
        
	\caption{Performance comparison between models without (marked in orange) and with the latent reconstruction.}
	\label{ReconstrutionComparsion} 
\end{figure} 


\section{Algorithm}
We provide the Pseudo-code of global alignment.
\begin{algorithm}[h]
\caption{Algorithm of Global Alignment}
\SetAlgoLined % Display line numbers if needed

\For{$x$ in $dataloader()$}{
    $x\_m \gets Mask(x)$\;
    $f\_m \gets OnlineEncoder(x\_m)$\;
    $f\_g \gets MomentumEncoder(x)$\;
    $f\_g \gets f\_g.detach()$\;
    
    $l\_pos \gets bmm(f\_m, f\_g.transpose(0,1))$\;
    $l\_neg \gets mm(f\_m, queue)$\;
    
    $logic \gets Cat(l\_pos, l\_neg)$\;
    $labels \gets Zeros(N)$\;
    
    $loss \gets CELoss(logic / \tau, labels)$\;
    
    $enqueue(f\_g)$\;
    $dequeue(f\_g)$\;
    $backward()$\;
    $momentum.update()$\;
}
\hrule
\vspace{2mm}
\scriptsize{\text{bmm}: batch matrix multiplication; \text{mm}: matrix multiplication;\\ CELoss: CrossEntropyLoss.}
%\text{cat}: concatenation.}
\end{algorithm}


\begin{table}
\centering
\small
\caption{Action recognition accuracy ($\%$) on the MSR-Action3D dataset. $\dagger$ indicates pre-training on NTU.}
\label{tab:msr}
  \begin{tabular}{l|c|c|c}
    \toprule
    
      Method & Reference &  Supervision & Accuracy \\
    \midrule
    MeteorNet~\cite{liu2019meteornet} & ICCV2019 & Supervised & 88.50 \\
    kinet~\cite{Zhong_2022_CVPR} & CVPR2022 & Supervised & 93.27 \\
    PSTNet~\cite{fan2021pstnet} & ICLR2021 & Supervised & 91.20 \\
    PPTr~\cite{wen2022point} & ECCV2022 & Supervised & 92.33 \\
    3DInAction~\cite{Ben-Shabat_2024_CVPR} & CVPR2024 & Supervised & 92.23 \\
    MAMBA4D~\cite{liu2024mamba4defficientlongsequencepoint} & CVPR2025 & Supervised & 92.68 \\
    P4Transformer~\cite{fan2021point} & CVPR2021 & Supervised & 90.94 \\
    PSTNet + PointCPSC~\cite{sheng2023point} & ICCV2023 & End-to-end Fine-tuning & 92.68 \\
    PSTNet + CPR~\cite{sheng2023contrastive} & AAAI2023 & End-to-end Fine-tuning & 93.03 \\
    PSTNet + PointCMP~\cite{shen2023pointcmp} & CVPR2023 & End-to-end Fine-tuning & 93.27 \\
    \midrule
    \rowcolor{gray!10}
    P4Transformer + MaST-Pre~\cite{shen2023masked} & ICCV2023 & End-to-end Fine-tuning & 91.29 \\
    \rowcolor{gray!30}
    \textbf{P4Transformer + Uni4D} & - & End-to-end Fine-tuning & \textbf{93.38} 
    \scriptsize (\textcolor{red}{+2.44}) \\  
    \rowcolor{gray!30}
    \textbf{P4Transformer + Uni4D$^\dagger$} & - & End-to-end Fine-tuning & \textbf{93.38} \scriptsize (\textcolor{red}{+2.44})\\
    \midrule
    \rowcolor{gray!10}
    P4Transformer + MaST-Pre~\cite{shen2023masked} & ICCV2023 & Linear Probing & 63.80 \\
    \rowcolor{gray!30}
    \textbf{P4Transformer + Uni4D} & - & Linear Probing & \textbf{84.62} \scriptsize (\textcolor{red}{+20.82}) \\ 
    \bottomrule
  \end{tabular} % 这里正确结束 tabular
\end{table}
